Calibration of Neural Networks

Neural networks solving real-world problems are often required not only to make accurate predictions but also to provide a confidence level in the forecast. The calibration of a model indicates how close the estimated confidence is to the true probability. This paper presents a survey of confidence calibration problems in the context of neural networks and provides an empirical comparison of calibration methods. We analyze problem statement, calibration definitions, and different approaches to evaluation: visualizations and scalar measures that estimate whether the model is well-calibrated. We review modern calibration techniques: based on post-processing or requiring changes in training. Empirical experiments cover various datasets and models, comparing calibration methods according to different criteria.

==> tabs/fl_ACC.tex <==
% \begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Датасет &            Модель &                     CE &                   FL 1 &                   FL 2 &                   FL 3 &                LS 0.05 \\
\midrule
    CIFAR-10 &       DenseNet121 & \textbf{94.92} &                  94.84 &                  94.90 &                  94.24 &                  94.52 \\
    CIFAR-10 &         ResNet110 & \textbf{94.82} &                  94.80 & \textbf{94.82} &                  94.70 &                  94.36 \\
    CIFAR-10 &          ResNet50 & \textbf{95.02} &                  94.58 &                  94.80 &                  94.52 &                  94.26 \\
    CIFAR-10 & Wide-ResNet-26-10 & \textbf{96.12} &                  95.70 &                  95.56 &                  95.64 &                  95.66 \\
   CIFAR-100 &       DenseNet121 &                  75.32 &                  75.66 &                  75.90 & \textbf{76.10} &                  75.54 \\
   CIFAR-100 &         ResNet110 &                  76.44 & \textbf{76.84} &                  76.74 &                  76.30 &                  75.96 \\
   CIFAR-100 &          ResNet50 &                  76.00 &                  76.38 &                  76.58 & \textbf{77.08} &                  76.18 \\
   CIFAR-100 & Wide-ResNet-26-10 &                  78.26 & \textbf{79.84} &                  79.64 &                  79.70 &                  78.14 \\
TinyImageNet &          ResNet50 &                  49.98 &                  50.10 &                  51.86 &                  51.06 & \textbf{53.62} \\
\bottomrule
\end{tabular}%
}
\caption{Accuracy, \% (больше -- лучше) -- доля правильных ответов без постобработки, столбцы соответствуют разным функциям потерь}
\label{tab:fl:ACC}
% \end{table}


==> tabs/fl_BS.tex <==
% \begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Датасет &            Модель &    CE &  FL 1 &                   FL 2 &                   FL 3 & LS 0.05 \\
\midrule
    CIFAR-10 &       DenseNet121 & 0.094 & 0.086 & \textbf{0.081} &                  0.089 &   0.102 \\
    CIFAR-10 &         ResNet110 & 0.097 & 0.086 & \textbf{0.082} &                  0.083 &   0.103 \\
    CIFAR-10 &          ResNet50 & 0.093 & 0.091 & \textbf{0.083} &                  0.085 &   0.102 \\
    CIFAR-10 & Wide-ResNet-26-10 & 0.069 & 0.070 &                  0.071 & \textbf{0.068} &   0.076 \\
   CIFAR-100 &       DenseNet121 & 0.446 & 0.385 &                  0.348 & \textbf{0.336} &   0.406 \\
   CIFAR-100 &         ResNet110 & 0.421 & 0.375 &                  0.358 & \textbf{0.346} &   0.386 \\
   CIFAR-100 &          ResNet50 & 0.411 & 0.365 &                  0.346 & \textbf{0.331} &   0.365 \\
   CIFAR-100 & Wide-ResNet-26-10 & 0.365 & 0.304 &                  0.287 & \textbf{0.281} &   0.326 \\
TinyImageNet &          ResNet50 & 0.677 & 0.648 & \textbf{0.620} &                  0.624 &   0.645 \\
\bottomrule
\end{tabular}%
}
\caption{Brier Score (меньше -- лучше) без постобработки, столбцы соответствуют разным функциям потерь}
\label{tab:fl:BS}
% \end{table}


==> tabs/fl_MCE.tex <==
% \begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Датасет &            Модель &    CE &                   FL 1 &                   FL 2 &                   FL 3 & LS 0.05 \\
\midrule
    CIFAR-10 &       DenseNet121 & 46.58 &                  36.54 & \textbf{27.80} &                  77.08 &   55.74 \\
    CIFAR-10 &         ResNet110 & 47.15 &                  73.35 &                  26.15 & \textbf{25.15} &   55.53 \\
    CIFAR-10 &          ResNet50 & 42.08 &                  37.23 & \textbf{25.00} &                  28.99 &   50.21 \\
    CIFAR-10 & Wide-ResNet-26-10 & 48.03 & \textbf{26.49} &                  33.49 &                  28.18 &   39.10 \\
   CIFAR-100 &       DenseNet121 & 54.14 &                  35.37 &                  26.13 & \textbf{14.76} &   46.99 \\
   CIFAR-100 &         ResNet110 & 58.32 &                  38.23 &                  30.27 & \textbf{25.44} &   40.00 \\
   CIFAR-100 &          ResNet50 & 47.19 &                  34.78 &                  23.83 & \textbf{14.00} &   31.28 \\
   CIFAR-100 & Wide-ResNet-26-10 & 55.83 &                  27.40 &                  16.16 &  \textbf{9.90} &   26.84 \\
TinyImageNet &          ResNet50 & 33.75 &                  18.63 &                   9.53 &  \textbf{6.39} &   26.59 \\
\bottomrule
\end{tabular}%
}
\caption{MCE, \% -- Maximum Calibration Error, (меньше -- лучше), 15 бинов без постобработки, столбцы соответствуют разным функциям потерь}
\label{tab:fl:MCE}
% \end{table}


==> tabs/fl_NLL.tex <==
% \begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Датасет &            Модель &    CE &  FL 1 &                   FL 2 &                   FL 3 & LS 0.05 \\
\midrule
    CIFAR-10 &       DenseNet121 & 0.422 & 0.230 & \textbf{0.186} &                  0.193 &   0.306 \\
    CIFAR-10 &         ResNet110 & 0.512 & 0.234 &                  0.195 & \textbf{0.185} &   0.301 \\
    CIFAR-10 &          ResNet50 & 0.428 & 0.253 &                  0.191 & \textbf{0.190} &   0.293 \\
    CIFAR-10 & Wide-ResNet-26-10 & 0.273 & 0.181 &                  0.161 & \textbf{0.158} &   0.224 \\
   CIFAR-100 &       DenseNet121 & 2.063 & 1.188 &                  0.948 & \textbf{0.903} &   1.435 \\
   CIFAR-100 &         ResNet110 & 1.843 & 1.165 &                  1.006 & \textbf{0.941} &   1.363 \\
   CIFAR-100 &          ResNet50 & 1.582 & 1.094 &                  0.951 & \textbf{0.897} &   1.230 \\
   CIFAR-100 & Wide-ResNet-26-10 & 1.437 & 0.898 &                  0.780 & \textbf{0.759} &   1.109 \\
TinyImageNet &          ResNet50 & 2.325 & 2.180 & \textbf{2.033} &                  2.038 &   2.334 \\
\bottomrule
\end{tabular}%
}
\caption{Negative Log-Likelihood (меньше -- лучше) без постобработки, столбцы соответствуют разным функциям потерь}
\label{tab:fl:NLL}
% \end{table}

